Backdoor Attacks in Peer-to-Peer Federated Learning

Most machine learning applications rely on centralized learning processes, opening up the risk of exposure of their training datasets. While federated learning (FL) mitigates to some extent these privacy risks, it relies on a trusted aggregation server for training a shared global model. Recently, new distributed learning architectures based on Peer-to-Peer Federated Learning (P2PFL) offer advantages in terms of both privacy and reliability. Still, their resilience to poisoning attacks during training has not been investigated. In this paper, we propose new backdoor attacks for P2PFL that leverage structural graph properties to select the malicious nodes, and achieve high attack success, while remaining stealthy. We evaluate our attacks under various realistic conditions, including multiple graph topologies, limited adversarial visibility of the network, and clients with non-IID data. Finally, we show the limitations of existing defenses adapted from FL and design a new defense that successfully mitigates the backdoor attacks, without an impact on model accuracy.

==> algorithms/bfs.tex <==
\begin{algorithm}[H]
\small

\KwData{Full Graph G, probability p, budget c}
%knowledge $\textsc{Agg}$}

\SetKwFunction{Diff}{Get Partial Observable SubGraph}

\SetKwData{rng}{rng}
\SetKwData{visibleBudget}{visible\_budget}
\SetKwData{visibleNodes}{visible\_nodes}
\SetKwData{queue}{queue}
\SetKwData{visitedNodes}{visited\_nodes}
\SetKwProg{Fn}{Function}{:}{}

\Fn{\Diff{$G, p, c$}}{
\BlankLine
\# create a random number generator\;
\rng $\leftarrow$ randomGenerator();

\BlankLine

\visibleBudget $\leftarrow$ numberNodes $\times$ c\;

\BlankLine
\# visible nodes\;
\visibleNodes $\leftarrow$ set()\;

\BlankLine
\# bfs queue\;
\queue $\leftarrow$ deque()\;


\BlankLine
\# bfs already visited nodes\;
\visitedNodes $\leftarrow$ set()\;

\BlankLine
\While{length(\visitedNodes) $<$ numberNodes \textbf{and} length(\visibleNodes) $<$ \visibleBudget}{
    \BlankLine
    \# choose the random node V\;
    random\_node $\leftarrow$ \choice(list(range(numberNodes)))\;

    \BlankLine
    \# random node is already visited\;
    \visitedNodes.add(random\_node)\;

    \BlankLine
    \queue.append((random\_node, 0))\;

    \BlankLine
    \# do bfs\;
    \While{length(\queue) $>$ 0}{
        \BlankLine
        \# pop the curr node with its depth from queue\;
        node, node\_depth $\leftarrow$ \queue.popleft()\;

        \BlankLine
        \# neighbours of node\;
        adjs $\leftarrow$ nx.neighbors(graph, node)\;

        \BlankLine
        \# traverse node's neighbors\;
        \ForEach{adj \textbf{in} adjs}{
            \BlankLine
            \# if adj already visited, ignore\;
            \If{adj \textbf{in} \visitedNodes}{
                \textbf{continue}\;
            }

            \BlankLine
            \# if depth is more than maximum, ignore\;
            \If{node\_depth + 1 $>$ d}{
                \textbf{continue}\;
            }

            \BlankLine
            \# generate a random value between 0 and 1\;
            random\_val $\leftarrow$ \rng.random()\;

            \BlankLine
            \# level visibility threshold, p\textasciicircum(d+1)\;
            threshold $\leftarrow$ p\textasciicircum(node\_depth + 1)\;

            \BlankLine
            \If{random\_val $\leq$ threshold \textbf{and} length(\visibleNodes) $<$ \visibleBudget}{
                \visibleNodes.add(adj)\;
                \queue.append((adj, node\_depth + 1))\;
            }

            \BlankLine
            \visitedNodes.add(adj)\;
        }
    }
}

\BlankLine
 \visibleNodes $\leftarrow$ list(\visibleNodes)\;
return \visibleNodes \;
}

\caption{Generation of Partial Observable subgraph $G'$}
\label{alg:partialObservability}
\end{algorithm}


==> sections/defense_v1.tex <==
% !TEX root = ../main.tex

\section{Defense\label{sec:defense}}
In this section, we  first introduce standard defenses against  poisoning attacks in FL and 
 show empirical evidence that these defenses are ineffective, slow down learning speed, and produce a final model with lower accuracy. We then show how to modify existing defenses to address specifics of the P2PFL setting and show that our defense can counteract backdoor attacks without a significant drop in model accuracy.

\subsection{Clipping Defense}
\label{sec:Clipping_Defense}
Gradient clipping is a standard defense against model poisoning and backdoor attacks against federated learning~\cite{sun2019can, gupta2021byzantine, hong2020effectiveness}. Since in FL learning clients are sampled to participate in rounds of training, the contribution of individual clients to the final model could be minimal. Still, adversaries can conduct model poisoning attacks where the contribution of each compromised node is amplified by the Boosting Factor applied to the local model. In the extreme, a model boosting attack could overwrite the global model, and therefore gradient clipping is critical to use to limit the contribution of individual clients.
%On one extreme, social media companies may only use a single client at most once during the training for adversarial robustness. That's why adversaries in FL and P2PFL can conduct a model poisoning attack because in a model poisoning attack contribution of each node is amplified by the Boosting Factor. The adversary might choose its boosting factor as big as the total number of nodes to make its contribution as big as the rest of the network. Since this attack vector is known, it is advised to deploy FL and P2PFL systems with Clipping Defense.  

In the gradient clipping defense in FL, the individual contribution of each participant is bounded by a threshold norm $C$ before aggregation is done at the server. We adapt this defense to the P2PFL setting. Instead of using  updates received from neighboring peers directly, a peer in P2PFL rescales each neighbor's update to fit within the maximum norm $C$ using equation~(\ref{eq:bound}).

\begin{equation}
    {U^{t}_j}_{clipped} = \frac{U^{t}_j}{max(1, \frac{|| U^{t}_j||}{C}) }
    \label{eq:bound}
\end{equation}

$U^{t}_j$ is the update sent by  peer $j$ at round $t$, $||U^t||$ is the $\ell_2$ norm of the client update, and $C$ is the clipping norm. Selecting  the clipping norm $C$ is not a straightforward task. Choosing a large $C$ would make the defense not effective. On the other hand, choosing it too small would slow down or stop convergence of the algorithm, similarly to choosing a very small learning rate.
One practical method for choosing $C$ is to simulate an experiment with only benign users and select $C$ based on their observed norm values. Also, $C$ is dataset-dependent, so this empirical procedure needs to be repeated for each new dataset. 

Clipping in P2PFL and FL differs significantly because in FL the server does not contribute to the learning protocol by producing its updates, but rather it aggregates the updates received from clients. On the other hand, in P2PFL, each node  participates by generating its local updates and aggregating them with the updates received  from the neighbors. The node can trust itself, so it is unnecessary to clip its own updates. However, when all other updates are clipped, and its own update is not, the peer starts to compute the next round's model mostly on its own update, which reduces the benefits of using P2PFL instead of local training. In a non-byzantine setting, clipping a node's model is equivalent to weighted averaging, where the weights for the local model and the neighboring models could be different.

We present results with clipping defenses in Figures~\ref{fig:defense1} a) and b). We selected clipping norm values of 1, 0.5, and 0.25 after running experiments and observing that norms for benign users are around 0.05,  and the local model's norm is around 3.5. For comparison, malicious users typically have norm values around 3.7 with our model boosting factor of 10. We first attempted to set the clipping value very close to 0.05, but the model did not converge with this small clipping norm. The figures show that the attack is still effective with 91\%, 83\%, and 72\% attack success for clipping norms 1, 0.5, and 0.25, respectively. Additionally, clipping slowed down the learning procedure dramatically: In all previous experiments 70 rounds were enough for models to fully converge, but with clipping defense, we increased the number of rounds to 200. Yet the increase in the number of rounds did not fully compensate for the loss in model test accuracy.  In Figure~\ref{fig:defense1} b), it can be seen that the model accuracy drops from 96\% to 91\%, 83\%, and 72\% for clipping norms 1, 0.5, and 0.25.


\subsection{Robust Aggregation Functions}
\label{sec:RobustAggregation}
Another standard method to defend against  poisoning attacks in FL is the application of robust aggregation functions. Robust aggregation function are designed for byzantine settings and have proven theoretical guarantees. Trimmed Mean, Trimmed Median, Krum, Multi-Krum, and Bulyan are known robust aggregation functions in the literature~\cite{KRUM, Bulyan,xie2018phocas}. These robust aggregation functions are designed for the central FL  setting, in which the server  receives updates from all users. On the other hand, in P2PFL, these algorithms must operate with partial information, given that nodes do not receive updates from all peers. We experimented with Trimmed Mean. In the Trimmed Mean, for each dimension of the vector, all peers updates are sorted, maximum and minimum $p$ values are excluded and the rest of the values are averaged. In our experiments, we used $p=1$, and we observed that Trimmed Mean is not effective against the backdoor attacks in P2PFL. Under the Trimmed Mean defense, the attacker still achieves 100\% attack success. 
Additionally, Trimmed Mean slows down the learning procedure, and we had to increase the number of rounds from 70 to 200 for convergence. Furthermore, in Figure~\ref{fig:trim}, it is shown that the Trimmed Mean defense decreases model test accuracy from 96\% to 83\% as a side-effect, while failing  to mitigate the attack.

\begin{figure}[ht]
    \centering   
    \subfloat[][Trimmed Mean Defense Test Accuracy ]{%
   \includegraphics[width=0.66\linewidth]{figures/TrimmedMean_bar_test_acc.png}}
    \caption{ Impact of Trim Mean Defense on Test Accuracy. The experiment runs on the Watts Strogatz graph with the EMNIST dataset, and 10\% percent of nodes (60) are malicious. The experiment uses the PageRank selection strategy. Results are an average of 3 trials and use the last round models (200th round). } 
    \label{fig:trim}
\end{figure}
\begin{figure*}[t]
    \centering   
    \subfloat[][Clipping Defense Attack Success ]{%
       \includegraphics[width=0.33\linewidth]{figures/Clipping_bar_attack_succ.png}}
    \subfloat[][Clipping Defense Test Accuracy]{%
       \includegraphics[width=0.33\linewidth]{figures/Clipping_bar_test_acc.png}}
    \subfloat[][Our Defense ]{%
       \includegraphics[width=0.33\linewidth]{figures/OurDefense_attack_succ.png}}
    \caption{ a) Effectiveness of Trimmed Mean Defense on Attack Success. b) Effectiveness of Trimmed Mean Defense on Test Accuracy. c) Effectiveness of our defense  on Attack Success. To measure the effectiveness of all these three defenses, experiments occur in one of the strongest attack vectors where 10\% of nodes are malicious, and the adversary uses the PageRank selection strategy. The experiment uses the Wattz Strogatz graph with 60 nodes and the EMNIST dataset. Results are an average of 3 trials and use the last round models (200th round). Experiments change their defensive strategy.}
    \label{fig:defense1}
\end{figure*}

\subsection{Our Defense}
\label{sec:OurDefense}
We showed in Section~\ref{sec:Clipping_Defense} that gradient clipping defenses are ineffective in the decentralized P2PFL setting. In the centralized FL setting, the  server does not contribute to the model updates, but in the P2PFL setting  each node trains a personalized model by receiving peer updates and a local model using the available local dataset.

For achieving adversarial robustness, it is natural to limit the contribution of each neighboring peer in the personalized model learned by a node. The clipping defense  decreases the contribution of each client, but if it is deployed similar to the centralized setting, it creates several issues.  If the clipping norm is too large for malicious nodes, the defense is not effective. If the clipping norm is too small for the local model, the convergence is significantly impacted. Due to these two limitations of a single norm value for clipping, we propose using two clipping norm values, one for bounding the neighbor peers' updates and one for the local model.
We have the flexibility to select a smaller norm for neighbor peers and a larger norm for the local model. We choose the neighboring norm as 0.1 and the local norm as 1 by considering that benign nodes typically have norm values of around 0.05 and the local model norm is around 3.5. In the Watts Strogatz graph, most of the nodes have  more than 10 neighbors. By setting the local model norm equal to 1, we will enable the local model to roughly have  equal impact to the rest of the network. This could be a limiting factor for some hard-to-learn tasks and non-iid data distributions. but we leave studying these problems for future work. 

In Figure~\ref{fig:defense1} c) we study the effectiveness of using two separate clipping norms as a defense strategy against poisoning. The attack success is 0\% percent, while model accuracy remains high at 96\%. Our two-norm defense is the only defensive strategy we are aware of that  provides effectiveness against backdoor attacks. Despite clipping requiring more rounds to converge, we observed that attack success increases with more rounds of training in Section~\ref{section:longTraining}, so our defense operates under a stronger setting for the attacker. Additionally, since the local model norm weighs the contribution of the local model and peer updates in real deployments, it can also be used as a configuration for the level of trust in the neighbors updates versus a node's own model. The defense can also be extended by using different weights for the neighboring peers, based on the level of trust a node has for its neighboring peer.  We leave this as an exploration for future work, in addition to testing the impact of poisoning attacks and defenses in peer-to-peer federated learning using other datasets and model architectures. 


==> sections/eval_v1.tex <==
% !TEX root = ../main.tex

\section{Experimental Evaluation}
\label{sec:evalution}
In this section we evaluate the effectiveness of the attacks presented in Section~\ref{sec:attacks}. We first introduce our methodology and show performance of our system under normal operation without attacks,
then evaluate the effectiveness of attacks and defenses under several settings. We seek to answer the following questions:
\begin{itemize}
\item What is the most effective strategy for the attacker to select nodes for the backdoor attacks?
\item What graph topology is more impacted by the attacks?
\item What is the impact of node robustness to failures on backdoor attacks?
\item How does training for longer impact the success of the attack?
\end{itemize}


\subsection{Experiment Setup}
\label{sec:Experiment_Setup}
{\em Network settings}. We use networks of 60, 80, and 100 peers.
Nodes are organized following a P2P network graph that defines how model updates propagate in the network.
We generated  three topologies that are commonly used in network science: Erdos Renyi, Watts Strogatz, and Barabasi Albert graphs, and model realistic network topologies. 

{\em Datasets.} We used the EMNIST and FashionMNIST adapted for P2P federated learning settings. Each dataset is partitioned into $n$ non-overlapping iid datasets, and each peer receives one of the datasets. We show the characteristics of the graphs we generated in Table~\ref{table:topology}.

{\em Attack Parameters.} The adversary chooses the following parameters: $k$, the number of malicious peers; Poison Data Ratio (PDR), the ratio of poisoned data over total samples in a malicious peer; boosting factor used in the model poisoning attack; adversarial training epoch count; and target class. We vary the $k$ values, while we fix PDR to 0.5, the boosting factor to 10,  adversarial training epoch count to 5, and the target class to 2. 

% PDR 0.5
% the boosting factor 10
% adversarial training epoch count 5
% target class 2

{\em Adversary node selection.} The adversary uses several strategies for  node selection, as described in Section~\ref{sec:identification_critical}. Specifically, the adversary uses random node selection as a baseline, and our four strategies based on maximum degree, maximum ENS score, maximum PagRank score,  and maximum clustering coefficient.
%by running graph algorithms, as described in Section \ref{sec:identification_critical}.

\begin{figure}[ht]
    \centering
        \caption{Network Topologies Used with $N=60$ nodes}  
        \subfloat[][Erdos Renyi]{%
       \includegraphics[width=0.33\linewidth]{figures/ErdosRenyi.png}}
    \subfloat[][Watts Strogatz]{%
       \includegraphics[width=0.33\linewidth]{figures/WattsStrogatz.png}}
    \subfloat[][Barabari Albert]{%
       \includegraphics[width=0.33\linewidth]{figures/BarabasiAlbert.png}}
       \label{fig:topology}
\end{figure}


\begin{table}[!htbp]
    \centering
\begin{tabular}{|l|r|r|r|r|}
\hline
name &  Erdos R. &  Watts S. &  Barabasi A.&  Complete \\
\hline
\# nodes         &        60.00 &                                 60.00 &            60.00 &     60.00 \\
\hline
\# edges         &       166.00 &                                360.00 &           576.00 &   1770.00 \\
\hline
Mean Degree      &         5.53 &                                 12.00 &            19.20 &     59.00 \\
\hline
Density          &         0.09 &                                  0.20 &             0.33 &      1.00 \\
\hline
Diameter         &         5.00 &                                  3.00 &             3.00 &      1.00 \\
\hline
Radius           &         3.00 &                                  2.00 &             2.00 &      1.00 \\
\hline
Mean Distance    &         2.56 &                                  1.88 &             1.68 &      1.00 \\
\hline
Transivity       &         0.10 &                                  0.24 &             0.39 &      1.00 \\
\hline
Clustering coef. &         0.09 &                                  0.24 &             0.41 &      1.00 \\
\hline
\end{tabular}
\caption{Characteristics of network topologies shown in Fig~\ref{fig:topology} }  
\label{table:topology}
\end{table}


All experiments used run for 70 epochs and  we repeated each experiment configuration with three different seeds. Results are averaged over the three runs. 

% node count

% 0.92692659,0.91241837,0.88421744

% fault-tolerance
% 0.92692659, 0.93800233,0.94894636,0.95949718

% graph type
% 0.96053613,0.92692659,0.8877813

\subsection{Performance without Attacks}\label{sec:no_attack}
In Figure~\ref{fig:baseline} we show the performance of our P2PFL system without attacks. As seen in the figure, our P2PFL system converges efficiently for networks with various node counts and graph types, and  it is resilient to node failures.

In Figure \ref{fig:baseline}a) we vary the size of the network from  60 to 100 nodes on the Watts Strogatz and EMNIST dataset, which are set as the default graph type and dataset for the rest of experiments. Model accuracy is 92\%, 91\%, and  88\% for the 60, 80, and 100  node graphs, respectively. Figure \ref{fig:baseline}b) presents results for the three  graph types we consider:  Erdos Renyi, Watts Strogatz, and Barabasi Albert with 60 nodes. Model accuracy is 96\%, 92\%, and  88\% for the Erdos Renyi, Watts Strogatz, and Barabasi Albert graph types, respectively. Figure \ref{fig:baseline}c) shows the model accuracy when  2, 4, or 6 nodes in the neighbour set of each peer crash, on the Watts Strogatz graph with 60 nodes, the default configuration.
Model accuracy is not affected negatively by the increase in the number of faulty nodes in the neighbor set in completely benign setting because the learning graph shifts from the Wattz Strogatz graph to the Erdos Renyi graph by removing some edges. In Figure~\ref{fig:baseline} b), we showed that model accuracy is higher in the Erdos Renyi. We observe a similar trend here by having 92\%, 93\%, 94\%, and  95\% for the 0, 2, 4, and 6 fault-tolerant setups, respectively.

\begin{figure*}[ht]
    \centering   
        \subfloat[][Node Count]{%
       \includegraphics[width=0.33\linewidth]{figures/Baseline_node_count.png}}
    \subfloat[][Graph Type]{%
       \includegraphics[width=0.33\linewidth]{figures/Baseline_graphtype.png}}
    \subfloat[][Fault Tolerance]{%
       \includegraphics[width=0.33\linewidth]{figures/Baseline_tolerant.png}}
       \caption{a) Impact of the number of nodes on test accuracy. The experiment varies N for values 60, 80, and 100. b) Impact of graph type on test accuracy. The experiment varies graph type for values Erdos Renyi, Watts Strogatz, and Barabasi Graph. c) Impact of r fault-tolerance. The experiment varies r for values 0, 2, 4, and 6. Unless the experiment varies the specific parameter of the experiment, it runs on the Watts Strogatz graph with the Emnist dataset, and all nodes are honest (k=0). There are 60 nodes (N=60). There are no failures r=0. } 
    \label{fig:baseline}
\end{figure*}
       
These three experiments suggest simpler graphs results in slightly better model accuracies. Erdos Renyi is the simplest graph, 60 is the graph with the least nodes so it is the simplest, and the 6 tolerant graph is the simplest. In the next sections, it will be shown that they are not the most resilient ones against attacks. 

\subsection{Attacker Node Selection}
\label{sec:selection} 

\textbf{Attacker node selection strategy.}
Figure~\ref{fig:attack1}a) measures the success of the attack under different selection strategies: random, maximum degree, maximum ENS, maximum PageRank score, and maximum clustering coefficient, which are introduced in Section~\ref{sec:identification_critical}. The experiment uses default values for graph type (Watts Strogatz), default node count (60), and default adversarial node percentage (5\%). The figure also evaluates attack success based on different hop distances as introduced in Section~\ref{sec:identification_critical}. The PageRank score outperforms other metrics and produces a 23\% improvement over the random attack. The maximum ENS score is the second best option with an 11\% improvement over the random baseline. The PageRank algorithm is even more effective with 27\% improvement over the baseline once we only consider nodes that have hop-2 distance. The second best method is again ENS, which provides a 13\% improvement over the baseline. In the rest of the attack experiments, we will consider only the PageRank selection strategy and comparing it against random selection. PageRank provides the best centrality score among the four metrics we evaluated, but  the random attack is still very effective, with 34\% attack success, and it does not require any previous knowledge or computation.
%We are considering PageRank because it has the highest improvement for the attack over the random selection strategy.We were expecting the PageRank to be successful up to a degree because the graph properties are similar to Web graph in terms of sparseness. Also, both tasks finding the most important website to list and the most important node to attack, are similar ordering goals because both aim to order the nodes based on importance. 

\begin{figure*}[ht]
    \centering   
        \subfloat[][Selection Strategy ]{%
       \includegraphics[width=0.33\linewidth]{figures/Selection_attack_succ.png}}
    \subfloat[][Adversarial Node Count ]{%
       \includegraphics[width=0.33\linewidth]{figures/adversary_count.png}}
    \subfloat[][Graph Type]{%
       \includegraphics[width=0.33\linewidth]{figures/GraphType_pagerank_attack_succ.png}}
       \caption{a) Impact of selection strategy on Attack Success. b) Impact of adversarial node count ($k$) on Attack Success.
       The experiment varies the selection strategy only on random and PageRank scores. c) Impact of the graph type on Attack Success. The experiment uses the PageRank selection strategy.  Unless the experiment varies the specific parameter of the experiment, it runs on the Watts Strogatz graph with the EMNIST dataset having 60 nodes (N=60) with three malicious nodes (k=3).} 
    \label{fig:attack1}
\end{figure*}


%\subsection{Impact of Number of Adversarial Nodes}\label{sec:adversarial_count}
\textbf{Number of adversarial nodes.}
\label{sec:adversarial_count}
Figure~\ref{fig:attack1} b)  varies adversarial node compromises between 1 and 6, for our default network of 60 nodes. The experiment uses the default graph (Wattz Strogatz), and default dataset (EMNIST). A PageRank selection strategy attacker achieves 41\% attack success by compromising 3 nodes (only 5\% of total nodes). Attack success reaches 98\% when the attacker compromises 10\% of all nodes. The random attacker performs worse, but is still effective for different levels of compromise. For instance, with a 5\% attack budget, the random attacker achieves 33\% success, and with a 10\% adversarial nodes budget, test accuracy increases to 92\%. The graph also shows that as hop-distance increases attack success decreases slightly. The hop-1 distance can be considered as the upper bound for the attack success from the adversarial distance perspective.



\subsection{Network Topology}\label{sec:topo}
\textbf{Impact of graph type.}
We now study the impact of the network graph on the attack. Specifically, we compare Erdos Renyi, Watts Strogatz, and Barabasi Albert graphs \cite{erdos1960evolution,albert2002statistical,watts1998collective}, demonstrated in Figure~\ref{fig:topology}. The properties of these graphs are included in Table~\ref{table:topology}. All these graphs are random and small-world graphs, Erdos Renyi has the least density in the number of edges, and Barabasi Albert has the most. These graph models are good representative models of  P2P graphs, such as  social media and cellular network graphs. Previous work suggests that P2PFL networks will most likely be small-world networks \cite{
martins2010hybrid,jiang2019new,dong2015experimental,liu2012distributed}.
Figure~\ref{fig:attack1} c)  varies network topology keeping all other aspects of the experiment setup fixed. The figure suggests as the model becomes  simpler, it becomes more prone to backdoor attacks. For example, in random selection strategy, attack success is 42\%, 34\%, and 23\% on Erdos Renyi, Watts Strogatz, and Barabasi-Albert graphs, respectively. The impact of graph type is considerably more important if the attacker can perform a PageRank algorithm for node selection as the attack success increases to  75\%, 42\%, and 41\% in the three graphs. 



\begin{figure*}[htb]
    \centering   

    \subfloat[][Impact of node count ]{%
       \includegraphics[width=0.33\linewidth]{figures/node_count.png}}
    \subfloat[][Dataset]{%
       \includegraphics[width=0.33\linewidth]{figures/Dataset_pagerank_attack_succ.png}}
    \subfloat[][Fault Tolerance ]{%
       \includegraphics[width=0.33\linewidth]{figures/Fault_tolerant_attack_succ.png}}
    \caption{ a) Impact of node count ($N$) on Attack Success. The experiment varies node count for values 60, 80, and 100 and 5\% percent of nodes are malicious. The experiment  uses  the random and PageRank selection strategies. b) Impact of the dataset on Attack Success. The experiment varies between EMNIST and FashionMNIST datasets. The experiment uses the PageRank selection strategy. c) Impact of fault tolerance  on attack success. The experiment varies robustness for values 0, 2, 4, and 6. Unless the experiment varies the specific parameter of the experiment, it runs on the Watts Strogatz graph with the EMNIST dataset having 60 nodes (N=60) with three malicious nodes (k=3) and no failures (r=0).} 
    \label{fig:attack2}
\end{figure*}

\textbf{Impact of network size.}
\label{section:NodeCount}
Figure~\ref{fig:attack2}a) varies the total number of nodes in the experiment to 60, 80, and 100 nodes. 
The experiment suggests that an adversary that can make a PageRank selection attack with a limited budget of adversarial nodes (5\%) is more effective on bigger graphs, which is not true for the random attacker. We  would also like to point out that keeping the malicious node percentage is very costly for attackers, for example, 5\% means three nodes out of 60 and five nodes out of 100 nodes. The adversary can achieve a much greater impact with 5 malicious nodes in 60 nodes (93\%) than in 100 nodes (46\%). This suggests larger graphs are more resilient against a fixed number of attackers but more vulnerable against the same ratio of attackers if the attacker can use graph algorithms for its placement strategy. 


\subsection{Impact of Dataset}
\label{section:Dataset}

Figure~\ref{fig:attack2}b) explores the extendibility of attacks on the Fashion MNIST dataset. Attack success is less than EMNIST, but the attack is still effective with 16\% success compared to the 42\% baseline in EMNIST. The experiment uses a moderate configuration. If the attacker's budget is increased to a higher number, we may achieve higher attack success. This result shows that our attack is a valid threat to other datasets. 

\subsection{Impact of Fault-tolerance on Backdoor Attacks}
\label{section:FaultTolerance}
As P2PFL is a collaborative and networked system, node failures are inevitable, and any P2PFL system should be tolerant to failures. In our fault-tolerant model, we assume failures happen randomly under the attacker's control.
Figure~\ref{fig:attack2} c) measures the impact of failures of neighboring nodes with varying the number of failed neighbors to 0, 2, 4, and 6.  As more neighboring nodes fail, the impact of the attack increases: For instance, the attack success without failures is 34\% and increases to 38\%, 41\%, and 50\% with 2, 4 and 6 node failures respectively. The clear trend in the graph suggests that an attacker can amplify backdoor attacks by crushing nodes in the P2P system.

\subsection{Impact of Longer Training}
\label{section:longTraining}
In our experiments, we varied the graph type, network size, and the graph fault tolerance capacity. These graph characteristics may potentially slow down or speed up model convergence since the learning process depends on these graph properties. For this reason, using a fixed round count of 70 for all the experiments might not be ideal, although models achieve more than 90\%  test accuracy at 70 rounds for our datasets. 

To evaluate the impact on the number of rounds, we repeated our experiments with 200 rounds, which is high enough to guarantee convergence on EMNIST. We analyzed attack success at rounds 110, 150, and 200, in addition to 70 rounds. Our experiments showed that running for longer has a positive impact on attack success. We observed that ENS becomes the most effective \textbf{node selection strategy} with 90\% attack success compared to  83\% attack success for PageRank at round $110$. After 150 rounds, all selection strategies achieve more than 94\%  attack success and their impact becomes similar. We observed that the attack gap among the \textbf{graph types} reduces when training for longer, and the attack reaches  100\%  success at round $200$ on all graph types. More specifically, the attack  reaches 99\%  success on Erdos Renyi graphs at round 110, and 83\% and 66\% success on Watt Strogatz and Barabasi Albert graphs, respectively. At round 150, the attack reaches more than 98\% success on  Erdos Renyi and  Watt Strogatz graphs, and 89\% on Barabasi Albert graphs.  We observed a similar pattern for \textbf{fault tolerance} as for graph types, as graphs with more fault tolerant capacity are more prone to attack, and the gap between them reduces with longer training. Precisely, the attack success we obtain is 69\%, 78\%, 82\%, and 94\% for 0-tolerant, 2-tolerant, 4-tolerant, and 6-tolerant graph models, respectively, at round $110$. At round $150$, 0-tolerant graphs obtain   94\% attack success, which increases to 100\% for 6-tolerant graphs. At round $200$, the attack reaches 100\%  success for all levels of fault tolerance. In addition, we observed that we need less \textbf{adversarial nodes} to achieve a similar attack impact. For instance, 3 attackers out of 60 total nodes (5\% attacker nodes) achieve more than 80\% and 90\% of attack success at rounds 110 and 150, respectively, compared to 42\% attack success at round 70.

%In 

%the pattern that simpler graphs are more prone to attack and

==> sections/evaluation/challenges.tex <==
\revision{\subsection{Implementation Challenges}}
\label{sec:Challenges}

%\revision{The experimental setup for simulating the P2P environment utilizes a virtual network of inter-connected Docker containers, all running concurrently on a single machine. Each container represents a peer in the P2P network, facilitating a realistic simulation of interconnected devices.}

\revision{The experimental setup for simulating the P2P environment utilizes a virtual network of interconnected Docker containers, all running concurrently on a single machine. Each container is configured to act as an independent peer within the P2P network, thereby enabling a realistic simulation of interconnected devices. The use of Docker containers allows for a controlled and consistent environment, ensuring that each peer operates with the same software and configuration settings. Additionally, running all containers on a single machine simplifies monitoring, allowing for the collection of comprehensive performance metrics and logs without the complexity of a distributed infrastructure.}

\revision{\myparagraph{Message Size} The complexity of the setup inevitably introduces certain challenges. Firstly, the efficiency of communication degrades as message size increases. As previously mentioned, communication between the peers is managed through GossipSub, a publish-subscribe messaging protocol, which effectively handles the dissemination of a large number of messages, mitigating the issue of network flooding. Amongst GossipSub's main design properties are \emph{reliability}, \emph{speed} and \emph{scale}, i.e. it must be able to handle a dynamically changing number of messages in an efficient and reliable manner. For simpler datasets such as MNIST, FashionMNIST, and EMNIST, small CNNs are sufficient, with model updates typically not exceeding 1MB. In contrast, more complex datasets like CIFAR-10 necessitate larger models with greater weight capacities, significantly increasing the size of communicated messages. To address this, an application-layer chunking mechanism is employed to divide the model updates into smaller chunks. These chunks are transmitted via GossipSub and reassembled at the destination node to reconstruct the original file.}

\vspace{3pt}

\revision{\myparagraph{Concurrency} The second challenge pertains to concurrency. Despite the host machine being equipped with two powerful GPUs, the Docker containers are unable to leverage GPU-backed training due to the necessity for mutual exclusion coordination among containers. This restriction limits the use of large and complex architectures, such as Residual Networks (ResNets) or VGGs.}

\vspace{3pt}

\revision{\myparagraph{Resources} The third challenge is related to memory constraints. Training a single model on the CIFAR-10 dataset centrally consumes approximately 2GB of RAM, encompassing pre-loading batches and data augmentation processes. Scaling this to a large number of nodes within the network is impractical. Our hardware is equipped with an Intel Xeon Silver 4114 CPU with 32 cores and 192GB of RAM. A network of 60 interconnected Docker containers, quickly exhausts the available memory, demonstrating the scalability issues inherent in this configuration.}


%We vary the $k$ values, while we fix PDR to 0.5, the boosting factor to 10,  adversarial training epoch count to 5, and the target class to 2. 

% PDR 0.5
% the boosting factor 10
% adversarial training epoch count 5
% target class 2

%All experiments used run for 70 epochs and  we repeated each experiment configuration with three different seeds. Results are averaged over the three runs. 


==> sections/evaluation/no_attack.tex <==
\subsection{Baseline Performance without Adversaries}
\label{sec:no_attack}

We begin our evaluation with the baseline performance of the P2PFL system, when no adversarial activities occur in the network. We find that the attack-free P2PFL system converges efficiently to classification accuracies generally well over 0.95 for various network topologies and network sizes, and is resilient to random neighboring link failures that cause missed model updates. 

\iffullpaper
These results are shown in Figure \ref{fig:baseline}. 
Figure \ref{fig:base_type} compares the test accuracy for the three graph types: Erdos Renyi, Watts Strogatz, and Barabasi Albert with 60 nodes. We observe that the test accuracy converges slower for the more complex networks. Thus, the small-world model of Watts Strogatz will take longer to converge compared to the Erdos Renyi random model, while the most complex model studied here, the Barabasi Albert scale-free network, will require the most number of rounds to converge. We note that all topologies will eventually reach very similar test accuracy, since the FL model is learned on the same training dataset (partitioned among peers). 

In Figure \ref{fig:base_size}, we vary the size of the Watts Strogatz network from 60 to 100 nodes. As expected, we see that the convergence speed decreases with network size, but the P2P federated learning model will eventually reach a similar test accuracy. 

Figure \ref{fig:base_ft} studies the fault tolerance of the P2P FL system on the Watts Strogatz configuration with 60 nodes. We vary the number of peer-adjacent connections that fail (i.e., 0, 2, 4, 6).  When more links fail, fewer peer updates affect the training process, hence the P2P FL model converges faster.
% However, given that the local training datasets have not changed, the system will eventually learn a similar machine learning model, capable of reaching similar test accuracy.

\begin{figure*}[ht]
    \centering   
    \subfloat[][Graph Type]{%
       \includegraphics[width=0.25\linewidth]{figures/Baseline_graphtype.png}
       \label{fig:base_type}
       }
    \subfloat[][Node Count]{%
       \includegraphics[width=0.25\linewidth]{figures/Baseline_node_count.png}
       \label{fig:base_size}
       }
    \subfloat[][Fault Tolerance]{%
       \includegraphics[width=0.25\linewidth]{figures/Baseline_tolerant.png}
       \label{fig:base_ft}
       }
       \caption{Baseline Performance (no attacks): a) Impact of graph type. b) Impact of network size. c) Impact of fault-tolerance (varying the number of missed model updates due to failed neighboring links). While these figures illustrate the first 70 rounds, our additional tests show that accuracy  will keep increasing as the training continues.} 
    \label{fig:baseline}
\end{figure*}

\fi

